Design Patterns for Situated Visualization in Augmented Reality

Situated visualization has become an increasingly popular research area in the visualization community, fueled by advancements in augmented reality (AR) technology and immersive analytics. Visualizing data in spatial proximity to their physical referents affords new design opportunities and considerations not present in traditional visualization, which researchers are now beginning to explore. However, the AR research community has an extensive history of designing graphics that are displayed in highly physical contexts. In this work, we leverage the richness of AR research and apply it to situated visualization. We derive design patterns which summarize common approaches of visualizing data in situ. The design patterns are based on a survey of 293 papers published in the AR and visualization communities, as well as our own expertise. We discuss design dimensions that help to describe both our patterns and previous work in the literature. This discussion is accompanied by several guidelines which explain how to apply the patterns given the constraints imposed by the real world. We conclude by discussing future research directions that will help establish a complete understanding of the design of situated visualization, including the role of interactivity, tasks, and workflows.

==> README <==
Created by Torsten Moeller, April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
modified by Bernhard Finkbeiner, July 5, 2010
modified by Tobias Isenberg, January 2016
modified by Filip Sadlo, March 2016
modified by Tobias Isenberg, July 2016
modified by Cagatay Turkay and Soumya Dutta, September 2019
modified by Cody Dunne, January 2022

This distribution provides a document class for formatting papers according to the specifications for submission to conferences sponsored by the IEEE Visualization & Graphics Technical Committee (VGTC).

Conferences that use the 'journal' document option:
- IEEE Visualization Conference (VIS)
- IEEE Virtual Reality (VR)
- IEEE International Symposium on Mixed and Augmented Reality (ISMAR)

It contains 13 files/directories:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default journal mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used with an established LaTeX environment by calling pdfLaTeX or LaTex. For online collaborative editing or without a local LaTeX installation, one option is to use https://www.overleaf.com/. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Unux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> notes/CHI2023-REVIEW.tex <==


Dear Dieter Schmalstieg,

Unfortunately, your paper: The Situatedness Continuum: A Design Space for Situated Visualization (number 2421) has been rejected from CHI2023. 

All papers that met a minimum threshold (at least one reviewer recommending: RR, Accept or RR, or Accept) have been put through to round 2. Any paper that did not receive at least one of these recommendations did not meet the threshold for entering round 2. This typically means that, although there could be merit for this paper in the future, reviewers thought that the paper could not be sufficiently improved within the five-week revise and resubmit period. Your reviews are below, and also will show in PCS in a few days. If you are interested in future publication, you could consider submitting to CHI2024 (or another conference) after making substantial changes to your paper.

CHI2023 received 3182 submissions. 234 papers (7.4%) were withdrawn or quick rejected before going out to review. 1530 (48.1%) received at least one R&R (or above) recommendation and were put forward to round 2. 1384 papers (43.5%) did not receive at least one R&R (or above) recommendation, and did not meet the threshold for entering round 2.

We wish you the best of luck with future submissions relating to this work.

Stefanie Mueller, Julie Williamson, and Max L. Wilson
CHI 2023 Papers Chairs


----------------------------------------------------------------

1AC review (reviewer 3)

  Expertise

    Expert

  Originality

    Low originality

  Significance

    Low significance

  Rigor

    Low rigor

  Recommendation

    I can go with either Reject or Revise and Resubmit

  1AC: The Meta-Review

    This paper proposes to extend the existing mixed reality and situated/embedded
    visualization models into a "situatedness continuum". The paper is mostly a
    theoretical or survey paper that discusses this extended design space, common
    design patterns, possible anti-patterns, and new designs.

    Score: The lion's share of this paper is the theoretical framework and the writing
    of the actual paper, but the reviews seem to indicate that the paper is still
    somewhat verbose, poorly structured, and hard to follow. Furthermore, there is
    substantial missing related work; beyond the citations named by the reviewers,
    surely the authors must be aware of Bressa's recent "What's the Situation with
    Situated Visualization?" survey. If so, it should have been cited and
    incorporated; if not, this points to a regrettable lack of awareness of current
    work in this field.

    In my view, the required changes here are too significant to be done in the space
    of the five-week CHI reviewing period. My recommendation is RRX. For future
    revisions, I recommend that they focus on restructuring and rewriting their paper.
    This will be a significant undertaking, however.

    The Good:
    + Useful and interesting extension of mixed reality and situated visualization
    (R1, R2, R4).
    + Taxonomy of situated visualization is valid (R1, R4).
    + The survey of the background is appropriate and useful (R1).
    + Timely and relevant work that builds and improves on previous work (R1, R4).

    The Bad: 
    - The work very clearly builds on previous work, and it is not always clear that
    this is not just incremental work (R1).
    - A fundamental assumption about the nature of immersive analytics seems invalid
    (R4).
    - The examples and design patterns are not internally consistent and rigorous
    (R4).
    - The paper is verbose and difficult to follow at times; more diagrams are needed
    (R1, R4).
    - The structure of the paper is somewhat chaotic (R1, R4).
    - No discussion of interaction; only on visual representations (R1).
    - The use of augmented reality is not always clear; some examples are from AR,
    some are not (R1, R4).
    - Also, what is the relation of VR to this space? (R2)
    - The continuum, design patterns, and examples are not always well-integrated into
    the argument (R1).
    - Much highly relevant work is missing (R2, R4).

----------------------------------------------------------------

2AC review (reviewer 4)

  Expertise

    Expert

  Originality

    Medium originality

  Significance

    High significance

  Rigor

    Low rigor

  Recommendation

    I can go with either Reject or Revise and Resubmit

  Review

    This paper introduces a way of analyzing situated visualizations in form of a so-
    called Situated Visualization continuum and strongly build on existing work by
    Willett et al. A design space is also proposed with both constraints and design
    variables, and potential applications are shown.

    This is an interesting paper which certainly addresses a timely topic. It is good
    that the authors attempted to further classify and systematically explore the
    space of situated visualizations. While the paper is comprehensibly written at the
    first glance, in many regards and details it is somehow confusing, less stringent
    and misses structure and scientific rigor. It is partly too verbose, needs to be
    improved in terms of English language, and relies too much on examples where there
    are different and contradictory opinions possible (I mention a few below). Many
    assumptions and terms are not clarified upfront, even what a (situated)
    visualization is (e.g., computer generated content or not).

    WRONG ASSUMPTION

    I have to disagree with the notion of the authors that Immersive Analytics means
    using VR headsets or other VR devices. This is not true, any kind of AR
    visualization is also considered a potential Immersive Analysis / Analytics
    application, and  there are quite a few research papers in that space. So, the
    sentence “… but usually do so in a purely virtual environment without any
    consideration of physical reality.” (124,125) really is wrong. Any kind of  AR
    visualization has to naturally take physical context into consideration, and any
    kind of AR visualization is able to produce a feeling of immersion. There are even
    papers devoted to investigating the relation between AR visualizations and the
    real environment, for example:

    Marc Satkowski and Raimund Dachselt. 2021. Investigating the Impact of Real-World
    Environments on the Perception of 2D Visualizations in Augmented Reality. In
    Proceedings of the 2021 CHI Conference on Human Factors in Computing Systems (CHI
    '21). Association for Computing Machinery, New York, NY, USA, Article 522, 1–15.
    https://doi.org/10.1145/3411764.3445330

    The distinction the authors make (and as it is written in several places) thus
    simply is a wrong assumption, and one should not build a paper on that.


    MISSING RELATED WORK

    While the background section is interesting to read and contains some very
    relevant papers, the cited 16 papers are far from being comprehensive in this
    larger and growing research area. Thus, I found it striking to see such a core
    paper like the following one on “Situated Analytics” not being considered and
    cited. This is a major flaw, not just a missing reference.

    N. ElSayed, B. Thomas, K. Marriott, J. Piantadosi and R. Smith, "Situated
    Analytics," 2015 Big Data Visual Analytics (BDVA), 2015, pp. 1-8, doi:
    10.1109/BDVA.2015.7314302.

    Other missing related work of quite some relevance:

    Vermeulen, J.; Collins, C.; Dachselt, R.; Irani, P.; Joshi, A. 2022. Reflections
    on Ubiquitous Visualization. In B. Lee et al. (Eds.), Mobile Data Visualization.
    Chapman and Hall/CRC, pp. 262-316, https://doi.org/10.1201/9781003090823-9

    Barrett Ens, Benjamin Bach, Maxime Cordeil, et al. 2021. Grand Challenges in
    Immersive Analytics. In Proceedings of the 2021 CHI Conference on Human Factors in
    Computing Systems (CHI '21). Association for Computing Machinery, New York, NY,
    USA, Article 459, 1–17. https://doi.org/10.1145/3411764.3446866

    G. Caggianese, V. Colonnese and L. Gallo, "Situated Visualization in Augmented
    Reality: Exploring Information Seeking Strategies," 2019 15th International
    Conference on Signal-Image Technology & Internet-Based Systems (SITIS), 2019, pp.
    390-395, doi: 10.1109/SITIS.2019.00069.

    N. A. M. ElSayed, R. T. Smith, K. Marriott and B. H. Thomas, "Blended UI Controls
    for Situated Analytics," 2016 Big Data Visual Analytics (BDVA), 2016, pp. 1-8,
    doi: 10.1109/BDVA.2016.7787043.

    M. Zheng and A. G. Campbell, "Location-Based Augmented Reality In-situ
    Visualization Applied for Agricultural Fieldwork Navigation," 2019 IEEE
    International Symposium on Mixed and Augmented Reality Adjunct (ISMAR-Adjunct),
    2019, pp. 93-97, doi: 10.1109/ISMAR-Adjunct.2019.00039.

    In addition, besides looking at the obvious terms, some work is closely related to
    the topics here and worth being considered, for example the “Augmented Display”
    concept (and related papers, see https://imld.de/augmented-displays/) being a form
    of hybrid user interface and display ecology likewise, also constituting a
    prominent example for parts of the situatedness continuum and contributing own
    systematics on alignment of physical referent (a display) and AR visualization
    (see subsection 5.4 of the submitted paper).

    Patrick Reipschläger, Severin Engert, and Raimund Dachselt. 2020. Augmented
    Displays: Seamlessly Extending Interactive Surfaces with Head-Mounted Augmented
    Reality. In Extended Abstracts of the 2020 CHI Conference on Human Factors in
    Computing Systems (CHI EA '20). Association for Computing Machinery, New York, NY,
    USA, 1–4. https://doi.org/10.1145/3334480.3383138


    THE VIEW CLASSES AND EXAMPLES – Contradictions and Ambiguities 

    In principle, I like the distinction into the four view classes and certainly
    appreciate the effort the authors make in describing them along with examples.
    However, I have to admit that, while reading, I several times disagreed with what
    is written. For example, if you argue the replicated views are a bit like a
    digital twin, the example of small multiples simply does not hold true and is a
    bad one in my opinion. Another example is the statement that the sub-views remain
    non-overlapping in the Aligned View class. There is the easily possible counter
    example of the gate sign being looked from above (e.g., a bridge) and overlapping
    the actual gate or a label overlaying the AR heart etc.

    Also, Figures 3 to 6 contain quite a number of arguable examples. What is, for
    example, the difference between an airport screen directly mounted on a post on a
    particular gate (here classified as aligned view) and a thermometer mounted on a
    stick in a steak (here classified as embedded view)? I cannot see one. Or, the
    Chameleon is conceptually similar to the medical labels in fig. 5 (they appear
    even more embedded to me than the Chameleon, which requires attention/view
    switches). Perhaps it is just my lack of understanding, perhaps the distinctions
    and differentiating criteria are less distinctive and clear than the authors
    assume (which would not be good for a comprehensive continuum). In addition, I
    wondered why none of the shown examples showcases a situated AR visualization. I
    could immediately cite a number of recent AR VIS / IA papers which would fit here
    very well. In general, I would have thought about visualization examples only, not
    static signage.

    I believe, one of the major problems the classification has is the notion of the
    secondary view. In some examples these are digital views (though you almost often
    exclude AR views, which I foremost had in mind while reading the paper), in others
    stationary displays like gate signage or thermometers. I would encourage the
    authors to more systematically make a distinction here and to provide better
    examples. For example, why not restricting yourself to any kind of digital/display
    secondary view? For me, a text label on a physical button is not much different
    than a “gate label” on a gate, and I do not consider this to be a “situated
    visualization”. Otherwise, the notion is too far-stretched.

    In addition, the concepts of a view region and world coordinate system need to be
    clearer introduced. Again, different interpretations are possible, and I was
    stumbling several times about what you wrote. For example, if you display an AR
    view aside a physical monitor, I would certainly classify this as an Aligned View.
    But they do not share the same camera transform – simply, since my eyes do not
    have a camera, nor does the physical monitor with content displayed. What means
    world coordinate system in this context? A coordinate system describing the real
    world? I admit getting confused with these notions, since they are not described
    upfront in a crystal clear way (if at all). Only in line 337 it is mentioned in
    passing that the eye of the user is the primary camera (which really is not a
    given concept…). What would be a “shared camera transform” if my eye is considered
    a camera?

    Another aspect coming to my mind is the possibility of further dividing / refining
    the last view class of embedded views. In my opinion, almost any AR HMD (or head
    /view-tracked mobile hand-held AR) based visualization falls into this category.
    So, if I am aiming at situated AR visualizations using an HMD – how does the
    entire continuum help me as a researcher or practitioner? Would there be
    meaningful sub categories?


    DESIGN SPACE

    The distinction between constraints and design variables seems meaningful to me. I
    find the descriptions partly too long-winding, repetitive and ambiguous, also
    concerning the examples (I particularly disliked the steaks example and found it
    not helpful; I also disagree with the Chameleon palmtop being an example for
    embedded views). If for example, one needs to explain so much on the simple
    concept of static or discrete location awareness, the concepts are either not good
    and clear enough or the readers not assumed to be intelligent enough to grasp
    them. Perhaps a better structured, more concise description would be helpful. It
    looks like time was not sufficient for a careful pass on these sections before
    submitting the paper.

    Concerning the navigation requirements (4.4) I thought that distance to the
    referent as well as viewing angle also play a central role and should be
    considered as constraints in the design space (they do not require navigation, but
    assume a static view point). So, perhaps “field of view” would be a better term.

    As a recommendation, perhaps the authors should think more about the later usage
    of the design space upfront. Sometimes, I rather had the feeling that
    justification was thought by explaining certain concepts and examples. How does
    the design space help me as an author without having to long think about in which
    of the categories falls my intended (or analyzed) concept? I am, for example, not
    sure whether it truly helps me as a visualization designer to think about the view
    class (5.1) in detail.

    Subsection 5.2 was rather weak in repeating well-known facts and excluding
    projections as a category. The projectors themselves might be static, but the
    projection dynamic/moveable (projected floor guidance for example); in addition,
    even though mobile projectors are not widespread, they should not be excluded in a
    scientifically comprehensive consideration.

    To conclude, the design space does not appear scientifically rigid enough to me
    (also, how the authors arrived there, which methodology they used to come up with
    these dimensions).


    APPLICATION & EVALUATION

    The authors directly jump into the idea of patterns, and I found this confusing
    and less convincing. “When studying the literature on AR” is also not a
    description of a thorough scientific methodology. In principle, it is a good idea
    to come up and describe design patterns. However, to add with the patterns yet
    another dimension to the continuum and the two design space parts did not convince
    me at all in terms of what a visualization designer can learn from it or how she
    will benefit from it. I could well imagine a systematic survey on AR visualization
    literature and the usage of the design space to classify the literature (or even
    to improve the proposes taxonomy).

    Also in the subsections 6.2 and 6.3 it largely remained unclear, how the continuum
    and the design space are *actually used*,  so which method was applied to arrive
    at the – again verbose – descriptions. I never felt informed about whether the
    treatment is comprehensible (e.g., is the list of design patterns complete?), and
    to just write (6.2) “It is easy to list several potential disturbing factors” is –
    with all due respect – not very scientific. Section 6.3, while touching many
    interesting topics, never goes into detail and is quite vague.

    Such a design space could be clearly evaluated as hinted above, e.g., by
    systematically considering  and analyzing existing literature with it, or by
    letting external designers/users use it to analyze existing solutions and compare
    the outcomes, or by letting people design novel situated visualizations and
    observe how they make use of it. None of this has happened to actually proof the
    benefits of this design space.


    SUMMARY

    In conclusion, this is certainly an interesting and timely (yet confusing) paper,
    which I could imagine eventually making interesting contributions, but which
    currently tries too much and lacks scientific maturity. For stronger contributions
    of value to the community, it needs to be far clearer in terms of assumptions
    made, relation to existing work, definition of terminology, describing the view
    classes, finding appropriate examples, being more systematic and scientifically
    rigorous. I am not sure whether the remaining five weeks will be enough time for
    the authors to turn this submission into a convincing and strong CHI publication,
    but would not object against a revise and resubmit.


    DETAILS

    -       The authors mostly used the more psychological term percept instead of
    perception, where the latter seems to be mostly more appropriate.
    -       The schematic visualization in figure 1 is difficult to understand
    (colors, text, role of rectangles, stippled pattern…). Try to find better visuals
    and describe them consistently.
    -       In the introduction to section 3, one could visually emphasize the four
    continuum classes that are described further down. This would enhance the reading
    experience
    -       387/88: I disagree with this sentence. A physical background with an
    overlaid AR visualization does not need to be a meaningful cognitive aid (see the
    CHI paper by Satkowski & Dachselt mentioned above).
    -	Fig. 3: QC code should be QR, I assume.
    -       Fig. 9: I disagree with navigation requirements simplified by these
    categories. A room, for example, can also contain obstacles where I have to move
    to look behind, not just in halls.
    -       Fig. 10: The table caption is too long, this should be part of the text.
    Also, I would expect far more visualization examples from the literature.

----------------------------------------------------------------

reviewer review (reviewer 1)

  Expertise

    Knowledgeable

  Originality

    Medium originality

  Significance

    Medium significance

  Rigor

    Medium rigor

  Recommendation

    I can go with either Reject or Revise and Resubmit

  Review

    Pros:
    + An interesting enhancement of current definitions of MR and SitViz
    + A valid taxonomy of SitViz design patterns
    + Strong background, with good links to popular definitions and their
    interpretations

    Cons:
    - A lot of concepts are an elaboration or adaptation of existing work, which
    somewhat masks the novelty of this work.
    - Quite verbose and difficult to follow at times. A lot of the information could
    be easier to understand diagrammatically
    - Tedious to link the parts of the paper - from the situated continuum to the
    design patterns.


    This work introduces the situatedness continuum, as means of defining a design
    space for situated visualization. The work is timely, as contemporary SitViz
    systems have been increasing in number, and researchers try to explore this space,
    driven by the increase of enabling H/W interfaces and related development
    ecosystems. Revisiting definitions, such as Milgram's continuum has been a
    recuring pattern of redefining work in the immersive domain. In this regard, this
    work will be of interest to the HCI community, given the popularity of immersive
    tech over the last few years.

    The proposed continuum focuses mainly on aspects of depiction and does not explore
    in depth the way we interact with these visualizations, once they are there.

    The authors state that their primary contribution, the continuum, lets a designer
    make a fine-grained decision concerning the integration of a visualization with
    the user's perception. I am not convinced that a designer's decision will be
    driven by such a framework - it may fit, or abide to the framework, but the
    decisions are surely dependent on the use-case and associated requirements.

    Although the proposed continuum has a lot of interesting aspects, I felt the
    narrative is quite verbose and difficult to follow. There are a lot of known
    aspects discussed whether in relation to HMDs or tracking, which often mask the
    different perspective offered by the authors. I feel the high reliance on text
    does not make it easy for the reader to see (and mentally classify) the different
    elements and taxonomies presented by the authors.

    Another issue is that the work at points jumps in and out of AR. For instance, the
    visualization patterns in Fig 12 are some interesting AR/MR usages. However,
    Figures 3 (all), Fig 5 (b), Fig.5(a)(c), and Fig.6 are not AR/MR. I found this
    generally confusing and distracting.

    In the background, the authors state that EWK determines how smart a SitViz
    appears - but what exactly does smart mean? Integrated to the environment?
    Realistic? Informative? Usable, indicative of the underlying information/data? The
    rest of the paragraph implies 'integrated' in my eyes, but I still feel it is a
    bit vague. For an SV to work, all of the above may apply.

    Section 3 should be separated in subsections, it is hard to follow through without
    them, possibly with each corresponding image in each section.

    On that note, Figures 3-6 are quite confusing in my eyes. Why would the departures
    screen be considered a situated view? Because they are situated somewhere?
    Likewise, the other two examples are just as confusing. Why would a QR-linked
    visualization of an online timetable is considered a situated visualisation?
    Because it refers to locations? That deviates a bit too far from previous
    definitions. I also appreciate the authors want to go beyond AR and include
    ambient displays etc - but that makes the concepts described quite convoluted.

    Likewise, I would agree with the 'replicated' characterisation of the Fig.4
    images, but there are some subtle differences between replicating the form (1st
    and 2nd), to providing annotations (3rd). Why is for instance the 3rd image not an
    aligned view (Fig 5. 2nd image).

    In terms of the design space constraints section, I think it is valid to consider
    them as design variables and constraints. These are considered well in the next
    two sections. Note, the recuring patters of Fig. 11 are actually 10, not nine as
    stated in the figure caption.

    Another issue I had with this work was linking things up, together. For example,
    in my initial read, it was unclear how does the situatedness continuum links with
    the design space, as section 5.1 is quite small, and the authors indicate that
    multiple view classes can be used in conjunction. Fig 10 does attempt to do that
    mapping, yet, besides a quite descriptive caption, it is not clear how does this
    mapping work, and requires a couple of re-reads. In this case, I would discuss
    Fig.10, early section 5 to highlight that mapping. In the same figure, it is
    unclear how the commonality of patterns was determined.

    In 5.5 the authors claim that their continuum considers visualizations that are
    located in 3D physical space, which may necessitate re-considering the benefits of
    3D visualization - without elaborating how this can be done.

    In section 6, the authors introduce a 'small, but distinct set of situated
    visualization patterns'. I must admit, it is unclear to me how these were
    determined (not that they are bad choices) and how where they named (less
    important). Was this through some form of analysis, or an expert opinion? What is
    the rational, say for trajectories when they could be connected glyphs? Some are
    also not referring necessarily to the depiction, but how it is seen. What stops is
    from having a magic lens and seeing glyphs in it (say in a zoomed map). With
    labels to inform us about each glyph. This could even be a proxy - say a focused
    view of an engine, zoomed in particular components with annotated glyphs to add
    context and info. I believe the issue here is that these patterns are not
    necessarily mutually exclusive - granted, this may not be the case in existing
    research where complex combinations have not yet been explored.

    Section 6.1 is another example of not being able to discern the mappings easily.
    The authors say that views in AR are mostly embedded, with three extension and
    three modification patterns, whereas the remaining views (aligned, replicated and
    situated) are mapped to a typical pattern. There is no elaboration of this, before
    the patterns are elaborated (independently of the view class).

    Moreover, it is difficult to compare the properties of these design patterns. I
    believe this could be summarised in a paper and make the information glanceable -
    and then elaborated with the current text. In fact, it is interesting to try to
    determine commonalities or differences (e.g., glyph vs decal vs ghost) but it is
    relatively hard at the moment. As a reader, I would need to sit down and make a
    comparison table myself, to provide a meaningful overview.

    Section 6.2 touches indirectly on interaction aspects with these patterns, but in
    many ways, it does not explore deeply how this is done, and its implications. I
    would agree that this may be a tad our of scope if the design patterns are
    restricted to 'depictions' but it does pose an interesting question, about how
    inclusive a design space may be, or whether it is doable to have such an all-
    inclusive design space in the first place.

    Finally, in terms of generation, I can see how a design space such as this can
    form a guidance framework, but beyond that what one does with SitVis is very much
    driven by the requirements at hand, rather than a set of rules that govern design
    and development.

    Overall, I found this paper very interesting, and it is definitely timely, and
    well-motivated work. However, I also found it difficult to navigate and extract
    high-level concepts. After reading it multiple times, I struggle to keep something
    that will assist me in work in SitVis and I would still return to prior, published
    work to scaffold my theoretical understanding in this domain. In this regard, I do
    not think this work is ready for publication, and it will require the paper to be
    effectively re-written, to do so.

----------------------------------------------------------------

reviewer review (reviewer 2)

  Expertise

    Expert

  Originality

    Medium originality

  Significance

    Low significance

  Rigor

    Medium rigor

  Recommendation

    I can go with either Reject or Revise and Resubmit

  Review

    The Situatedness Continuum: A Design Space for Situated Visualization

    This paper introduces several concepts and dimensions for a design space to cover
    'situated visualization', in which
    real and virtual content are displayed together. The design space is intentended
    to cover
    common design patterns, to critique situated designs, and to generate new designs.

    This paper provides some valuable insights into the design challenges around
    augmenting user views with supplemental digital information.
    It would be strengthened by including prior work, especially considering user
    perception and taxonomies of the coordinate systems
     
    A design space must cover all existing examples AND suggest new ones with mutually
    exclusive dimensions.
    In this sense, Figure 10 (really a table) and Fig 12 are nice 

    Figure 9 makes navigation look like a virtual environment, even suggesting a CAVE.
    ?


    While Milgram et al.’s classification of mixed reality systems is
    a useful starting point to structure and discuss the design space
    of Mixed Reality and Mirror Worlds, we find that it does not address
    some key aspects of interaction and display...  Fig 2 is OK.

    A simple 2x2 model was proposed in Polys NF, Knapp B, Bock M, Lidwin C, Webster D,
    Waggoner N, Bukvic I. Fusality: an open framework for cross-platform mirror world
    installations. InProceedings of the 20th international conference on 3D web
    technology 2015 Jun 18 (pp. 171-179).

    The Skarbez work is well taken, and may be more important if the authors consider
    this proposed design space from a user-centered point of view (user perception is
    primary).
     
     
    Some important suggestions to consider in this proposed taxonomy / design space:

    'Situated Visualizations' in the authors' definition requires the user to be
    situated in the real/physical world.
    However, virtual worlds can provide similar perceptual properties to the real
    world
     ... (one can simulate AR in VR, but not vice versa!).

     This fact is a missed opportunity for the authors to consider how access,
    navigation, and perception generally
     in Information-Rich Environments (IREs). 
     
     This same graphical challenge has been definied and explored before as
    Information-Rich Virtual Environments (IRVEs), Where
     'abstract' information is portrayed in a visualziation in conjuntion with the
    'perceptual' information that is apparent in the physical world:

    Bowman DA, North C, Chen J, Polys NF, Pyla PS, Yilmaz U. Information-rich virtual
    environments: theory, tools, and research agenda. InProceedings of the ACM
    symposium on Virtual reality software and technology 2003 Oct 1 (pp. 81-90).


    The coordinate system and relation of visualization to the referent are indeed
    crucial aspects when one considers the human perception
    of Depth cues and Gestalt cues provided by a visualization. Indeed, Polys
    developed a design space in this area, specifically about the relation of
    supplemental
     'abstract' information to its referent by the congruety of depth cues and
    association cues between them.
     
    In that work, he related the value of information shown in these layout spaces to
    different user tasks and to different displays
    through human-subjects experiments with text label layout algorithms:

    Polys NF, Bowman DA, North C. The role of depth and gestalt cues in information-
    rich virtual environments. International journal of human-computer studies. 2011
    Jan 1;69(1-2):30-51.

    Polys NF, Kim S, Bowman DA. Effects of information layout, screen size, and field
    of view on user performance in information-rich virtual environments.
    InProceedings of the ACM symposium on Virtual reality software and technology 2005
    Nov 7 (pp. 46-55).

    In those experiments, he also considered aspects of clutter and how dynamic
    layouts can be used in conjunction with user navigation.

    These works would be important to situate in a full accounting of this design
    space.


    Finally to make this less of a survey paper, it would be valuable to provide more
    treatment of the evaluation and generation aspects. In the first case, this would
    be pointing to studies that compared different points in the design space; in the
    second, it would propose some new possibilities and designs.

----------------------------------------------------------------



==> notes/ben-notes.tex <==
09-03-2023 Things to do:
1. Exclude the ProxSituated paper
    - We no longer consider it to be in scope due to the myriad variables that it introduces
    - Establish early on that we are looking at situated AR situations with actual physical referents as per the definition of Willett et al.
    - Our design space may potentially act as a basis for a future prox-situated design space
2. Split the location variable into two
    - One would be for accuracy of the view: does it relate to a specific part of the referent?
    - The other would be for the alignment of the view: this might be the original view classes.
3. Remove immediateness
4. Add a diagram to explain view cardinality better
5. Expand on the limitations of the design space and how they are future work



















- What exactly is the contribution and novelty here? 
    - The situated continuum essentially re-classifies the original ideas from Willett et al.'s Embedded Data Representations paper 
        - Replicated views are already talked about under Section 6.4 Facsimiles
        - Aligned and embedded views all fall under the general bucket of embedded visualisations
    - There's not really a need yet to classify and taxonimise 
        - The continuum is essentially doing this, but it feels wholly unnecessary 
        - The act of classification is useful if you can generalise design guidelines to everything in the class, but this paper doesn't even do this 
        - The view classes should be born out of design space dimensions (much like the design patterns), not the other way around 
    - It's not clear how a designer would use this work 
        - Not many new or exciting ideas are provided 
        - No clear actionable steps, where to begin in the design space 

- The notion of identifying design patterns in situated visualisation could be promising 
    - The Bressa et al. survey paper has already done a little bit of this, by identifying six case studies 
- We could also dive a lot deeper into the "levels of indirection" of Willett et al.
    - That's almost what the continuum and design space are anyway
        - It considers factors like the spatial directness between physical and virtual views, the alignment of the two, etc.
    - What this would essentially be is to create design levers that can affect the design of a situated visualisation
    
- Perhaps this is where we reverse the entire paper around
    - Start with design patterns based on a light literature survey. We identify what are some common designs and characterise them
    - Next, we identify a set of design variables that further characterise these design patterns. Theoretically, this will be generative as adjusting any variable will still create some form of design, irrespective of its legibility or not
    - We can then plot the initial design patterns onto these design variables. Depending on the number of variables, we can loosely characterise different parts of these variables into classes, in the same way that the continuum currently does
    - And then, we can introduce the constraints as factors which designers need to consider when designing situated visualisation
    - Lastly, we characterise specific works (maybe the six exemplars in Bressa et al.) using our patterns, design space, and view classes
    - This will have a much stronger design lens, making its practicality for creating new designers clearer. It also gives less of an impression of taxonimisation, and more of one about ideation and generation
















% OLD...

Section specific changes:
- Section 1: Introduction
    - Rewrite using the following flow:
        1. Immersive headsets have recently been used to bring data into the space around users. In the case of VR applications, the focus is solely on the virtual artefacts and the interactions they afford
        2. In contrast, AR applications take place in the physical world, allowing for strong semantic relationships between the physical and the virtual, also known as situated visualisation
        3. The design of the virtual views w.r.t. the physical environment plays a crucial role in these applications. Digital information oftentimes needs to be associated with physical objects (or referents). The most common approach is to leverage the Gestalt law of proximity: placing the virtual view as close to its physical referent as possible in space.
        4. This concept is exemplified by Willett et al. and embedded visualisations, which present information directly overlaid on top of the physical object.
        5. This is not always desirable however. Due to factors such as clutter and occlusion, it may be instead beneficial to place virtual views close to the referent to establish a clear semantic relationship, but far enough to ensure visibility and usability.
        6. From this, we can devise a continuum of levels of proximity (or ``situatedness'') in which the virtual view has with the physical referent. This continuum then forms part of a larger design space for how situated visualisations may be designed.
        7. Such a design space however is constrainted by technological and contextual factors (see Bressa et al.) that must be considered by the situated visualisation designer.
        8. We therefore contribute:
            - A design space and continuum for situated visualisation
            - A set of constraints that must be considered when designing situated AR applications
            - An example gallery characterising prior work using the design space and continuum
            - A series of guidelines for how the design space and continuum can be used
- Section 2: Related Work
    - Add subsections on the following topics:
        - Augmented reality and immersive analytics
        - Situated visualisation
        - Design spaces and taxonomies
    - Move a lot of the works which are used to argue for the design space into either the design spaces and taxonomies subsection, or into the design space section itself
- Section 3: Situatedness Continuum
    - Change a lot of the analog examples to AR examples
    - Adjust the definition of replicated views.

==> notes/ben-suggested-changes.tex <==
\section{Ben's suggested changes}
The two main problems of this paper are:
\begin{itemize}[noitemsep]
    \item It is barely written from a design perspective, focusing too much on technical definitions and classification
    \item The different contributions rarely build upon each other and are not cohesive
\end{itemize}

To solve this, I suggest we flip the entire paper on it's head---we reverse the flow starting from the design patterns, putting the design first.

The structure would be something as follows:
\begin{enumerate}
    \item Introduction
    \item Related work
        \begin{itemize}
            \item The most important works here are probably Willett et al.\ \cite{Willett2017} and Bressa et al.\ \cite{Bressa2022}
            \item Key concepts from Willett et al.\ \cite{Willett2017} are: partitioning data and referents into sub-presentations; classes of data representations (non-situated, situated, embedded); inclusion of physicalisations; levels of indirection (spatial and temporal); use of facsimiles as stand-ins for referents
            \item Key concepts from Bressa et al.\ \cite{Bressa2022} are: their summary of findings from their survey (i.e. limited engagement with definitions, data representations, and target audience. Focus on AR as a technology. Focus on spatiality); six exemplars to characterise the entirety of situated visualisation; new perspectives on space, time, place, activity, and community; discussion on technological considerations
        \end{itemize}
    \item Design patterns in situated visualisation
        \begin{itemize}
            \item We can probably reuse most of the existing patterns
            \item Specify which works these specific patterns came from
        \end{itemize}
    \item Design space and dimensions
        \begin{itemize}
            \item We can take some aspects of the existing design space (e.g. alignment)
            \item We can also introduce new ones (e.g. extent of data partitioning a la Willett et al. \cite{Willett2017})
        \end{itemize}
    \item View classes
        \begin{itemize}
            \item In the best case scenario, we take our design dimensions, and then draw out regions of the n-dimensional space which correspond to the view classes
            \item These view classes would more or less be similar to the existing ones, although with perhaps some added ones
            \item This does remove the notion of the continuum, but the definitions can be a lot more "fuzzy" and therefore not rely on hard computer graphics-like criteria such as view transforms
        \end{itemize}
    \item Application to existing exemplars
        \begin{itemize}
            \item We can characterise our design space and view classes by applying them to existing examples
            \item Bressa et al.\ \cite{Bressa2022} includes several examples that would be good to reuse
        \end{itemize}
    \item Discussion and design recommendations
    \item Conclusion
\end{enumerate}

There are several topics that have come up in related work which were not in this paper's original version, but we might want to include. Excluding these would make them limitations:
\begin{enumerate}
    \item Do we focus solely on AR or do we include physicalisations?
    \item Do we consider interactivity at all?
\end{enumerate}

==> notes/design-space-ideation.tex <==
SITUATED VISUALISATION PIPELINE
Before even designing the visualisation itself, the designer needs to factor in a set of constraints that they have to deal with. Constraints are hard limitations that are imposed onto the designer that affect their ability to even implement the designs. These are either technological or contextual constraints. These constraints are especially important as the real world is full of constraints.

a) The extent of world knowledge that the application has of the referents and their properties
    - This may limit the data available
b) The extent of location awareness of the application
    - This may affect the ability for embedded views
c) Navigational requirements of the application
    - This may affect the visibility of the views
d) Size and accessibility of the referent(s)
    - A proxy of the referent may need to be used

Note that referent arrangement is not necessarily a constraint, as the designer can design around it by choosing to aggregate instead of using a view per referent. This is more of a design consideration since the arrangement doesn't force the designer to use a certain view.

Then the designer needs to consider the relationship between the data and referent.
a) What is the cardinality between the data and referent?
    - One-to-one: one row of data values relates to one single referent
    - Many-to-one: many rows of data values are related to a single referent
    - One-to-many: one row of data values is represented by multiple referents
    - Many-to-many: many rows of data values are each represented by their own referent
        - In cases where multiple referents are used, it is important to consider whether or not it is necessary to see all referents simultaneously (e.g. to observe a trend). If a hard navigational requirement is to have multiple fields of regard, it may be necessary for the designer to use a single view instead of separated views.
b) What type/class of information is to be shown?
    - Tabular information: data that can be encoded using visual channels
    - Relational information: data that shows relationships between entities
    - Structural information: data relating to 3D structures and objects
c) What level of spatial granularity is there between the data and parts of the referent?
    - High granularity: The data is associated with specific spatial points on the referent
    - Medium granularity: The data is associated with specific spatial regions on the referent
    - Low granularity: The data is associated with the entire referent as a whole
d) What level of temporal indirectness is there between the data and the referent?
    - High indirectness: The data is either delayed or forecasted from the events occurring on the referent
    - Low indirectness: The data is updated almost instantaneously from the events occurring on the referent
    - No indirectness: The data is completely static and does not change over time.

Lastly, the designer can choose how to present the information in the context of the referent.
Option a) Modify the referent
    - Directly change the appearance of the referent itself by modifying its shape, texture, or colour
    - This can be thought of directly embedding information into the referent itself, or using the referent as the visualisation
    - Applicable patterns are decal, shape change, and lens
Option b) Extend the referent
    - Add additional visual information to the referent using discrete glyphs
    - In the original paper's nomenclature, this can be thought of as aligning glyphs along the referent
    - Whether or not this spatial alignment conveys information depends on the spatial granularity listed above
    - Applicable patterns are glyph, ghost, trajectory, and label
Option c) Complement the referent
    - Place the data in spatial proximity to the referent
    - This is more or less what a situated visualisation is
    - Applicable patterns are mirror, proxy, and panel


DESIGN VARIABLES
These design variables are mostly repeats of the above questions, as the pipeline ultimately considers the design space variables. The pipeline also provides a more structured way at looking at these variables, particularly with respect to the data.

a) Spatial position: Where is the view placed on the referent?
    - Points: onto specific parts of the referent
    - Regions: onto a large region of the referent
    - Whole: onto the entire referent
    - Aligned: aligned against the side of the referent
    - External: completely separate from the referent
b) Duplicity: How is the view divided across the referents?
    - Singular: the view is on or nearby a single referent
    - Multiples: the entire view composed of small multiples which each represent a subset of data (e.g. a pie chart showing a breakdown of manufacturing costs for each product)
    - Separated: the entire view is separated and spread out across all referents (e.g. mapping colour to the cost of materials for each product)
    - Duplicated: the entire view is duplicated exactly across multiple referents
c) Visibility: Under what conditions can the view be seen?
    - Occluded: view follows regular rules for occulusion just like a real object
    - Toggle: view is toggled on and off manually by the user
    - Focus: view appears when the referent is in focus, by picking it up, looking at it, etc.
    - Proximity: view appears when in close proximity to the referent
    - Always visible: view is always visible regardless of occlusion
d) Immediateness: Is the referent the actual referent itself? (from \cite{satriadiProxSituatedVisualizationExtended2023})
    - Immediate physical referent: The referent used is the actual referent
    - Proxy referent: The referent used is a (virtual) proxy of the referent
    - Mixed: Both actual referents and proxy referents are used


Note that we intentionally exclude design variables that have to do with visual channels such as colour, shape, orientation, etc.


SPATIAL AND TEMPORAL INDIRECTION
These concepts would largely sit outside of the design space, but can be used to comment on the design space. Temporal indirection largely exists separately from the design space I think, as it mostly informs the design choices and not necessarily is a design choice itself.

TRANSITIONS ACROSS DIFFERENT SITUATED VISUALISATIONS
Willett et al. talkes about this. We can describe how the design space can be used to generate equally valid situated visualisations at different levels of embeddedness. Some way to transition between these would then need to be explored in the future.

COMPOSITE VISUALISATIONS
A situated visualisation may be composed of multiple patterns. It may be that it is advantageous to double encode data by presenting it in two different ways, or in two levels of aggregation. It may also be advantageous to display two different types of data on the same referent, such as showing a decal on a ghost extension of a referent.
